Unmixing methods based on nonnegativity and weakly mixed pixels for astronomical hyperspectral datasets

[Abridged] An increasing number of astronomical instruments (on Earth and space-based) provide hyperspectral images, that is three-dimensional data cubes with two spatial dimensions and one spectral dimension. The intrinsic limitation in spatial resolution of these instruments implies that the spectra associated with pixels of such images are most often mixtures of the spectra of the "pure" components that exist in the considered region. In order to estimate the spectra and spatial abundances of these pure components, we here propose an original blind signal separation (BSS), that is to say an unsupervised unmixing method. Our approach is based on extensions and combinations of linear BSS methods that belong to two major classes of methods, namely nonnegative matrix factorization (NMF) and Sparse Component Analysis (SCA). The former performs the decomposition of hyperspectral images, as a set of pure spectra and abundance maps, by using nonnegativity constraints, but the estimated solution is not unique: It highly depends on the initialization of the algorithm. The considered SCA methods are based on the assumption of the existence of points or tiny spatial zones where only one source is active (i.e., one pure component is present). In real conditions, the assumption of perfect single-source points or zones is not always realistic. In such conditions, SCA yields approximate versions of the unknown sources and mixing coefficients. We propose to use part of these preliminary estimates from the SCA to initialize several runs of the NMF to constrain the convergence of the NMF algorithm. Detailed tests with synthetic data show that the decomposition achieved with such hybrid methods is nearly unique and provides good performance, illustrating the potential of applications to real data.

==> abstract.tex <==
An increasing number of astronomical
instruments (on Earth and space-based) provide hyperspectral images, i.e. three-dimensional
data cubes with two spatial dimensions and one spectral dimension. The intrinsic limitation 
in  spatial resolution of these instruments implies that the spectra associated with pixels 
of such images are most often mixtures of the spectra of the ``pure'' components
that exist in the considered region. In order to estimate the spectra and spatial abundances 
of these pure components, we here propose an original Blind Source Separation (BSS),
i.e. unsupervised unmixing, method. Our approach is based on extensions and combinations of
linear BSS methods belonging to two major classes of methods, namely
Non-negative Matrix Factorization (NMF) and Sparse 
Component Analysis (SCA). NMF performs the decomposition 
of hyperspectral images, as a set of pure spectra and abundance maps, by using
non-negativity constraints, but the estimated solution is not unique: 
it highly depends on the initialization of the algorithm. 
The considered SCA methods are based on the assumption of the existence 
of points or tiny spatial zones where only one source  is active
(i.e., one pure component is present). These  points or zones are 
then used to estimate the mixture and perform the decomposition. In real 
conditions, the assumption of perfect single-source points or
zones is not always realistic. In such conditions, SCA yields approximate
versions of the unknown sources and mixing coefficients.
We propose to use part of these preliminary estimates from the SCA to initialize
several runs of the NMF, in order to refine 
these estimates and further constrain the convergence of the 
NMF algorithm. The proposed methods also estimate the
number of pure components involved in the data and they provide error
bars associated with the obtained solution. Detailed 
tests with synthetic data show that the decomposition achieved with 
such hybrid methods is nearly unique and provides good performance, 
illustrating the potential of applications to real data. 

 
